An improved method for solving quasilinear convection diffusion problems on a coarse mesh

A method is developed for solving quasilinear convection diffusion problems starting on a coarse mesh where the data and solution-dependent coefficients are unresolved, the problem is unstable and approximation properties do not hold. The Newton-like iterations of the solver are based on the framework of regularized pseudo-transient continuation where the proposed time integrator is a variation on the Newmark strategy, designed to introduce controllable numerical dissipation and to reduce the fluctuation between the iterates in the coarse mesh regime where the data is rough and the linearized problems are badly conditioned and possibly indefinite. An algorithm and updated marking strategy is presented to produce a stable sequence of iterates as boundary and internal layers in the data are captured by adaptive mesh partitioning. The method is suitable for use in an adaptive framework making use of local error indicators to determine mesh refinement and targeted regularization. Derivation and q-linear local convergence of the method is established, and numerical examples demonstrate the theory including the predicted rate of convergence of the iterations.

==> makefile <==
#! make
##############################################################################
# Purpose: MCP (Mathematical and Computational Physics Group) paper makefile.
#
# Notes:   This makefile is used by the MCP group (Michael Holst's Research 
#          Group in the Mathematics and Physics Departments at UC San Diego)
#          to build latex papers using the fairly simple combination of 
#          pdflatex, amstex/amslatex, and pdf/png images.
#
# Targets: The makefile will auto-generate the following based on the
#          requested make target:
#
#            Main Targets:
#
#              pdfth   --> ${TARGET}.pdf via pdflatex
#              pdf     --> ${TARGET}.pdf via pdflatex + thumbpdf
#              dvi     --> ${TARGET}.dvi via latex
#              dvip    --> ${TARGET}.dvi|ps|pdf via latex + dvips + ps2pdf
#
#            Auxilliary Targets:
#
#              arx     --> zarxiv.tar.gz (gzipped tarball for arXiv)
#              clean   --> rm -f *.aux, *.dvi, etc
#              rclean  --> clean + rm *.ps *.bbl (careful!)
#              rrclean --> rclean + rm m.pdf mm.pdf ${TARGET}.pdf (careful!)
#
# Author:  Michael Holst
# Date:    Sat Dec 19 22:23:18 PST 2009
##############################################################################

default: pdf

TARGET=arXbTRN15a

ARXIV_DIR=zarxiv
ARXIV_FILES=${TARGET}.tex ${TARGET}.bbl \

LATEX=latex
PDFLATEX=pdflatex
#PDFLATEX=pdflatex --shell-escape
BIBTEX=bibtex
#BIBTEX=./zbibtex

all : pdf arx

dvi :
	make clean
	${LATEX} ${TARGET}.tex
	-${BIBTEX} ${TARGET}
	${LATEX} ${TARGET}.tex
	${LATEX} ${TARGET}.tex
	-cp -f ${TARGET}.dvi mm.dvi

dvip : dvi
	dvips -N0 -P pdf -t letter -o ${TARGET}.ps mm.dvi
	ps2pdf ${TARGET}.ps
	-cp -f ${TARGET}.pdf mm.pdf

pdf :
	make clean
	${PDFLATEX} ${TARGET}
	-${BIBTEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	${PDFLATEX} ${TARGET}
	-cp -f ${TARGET}.pdf mm.pdf

pdfth : pdf
	thumbpdf ${TARGET}
	${PDFLATEX} ${TARGET}
	rm -f thumb*.png
	-cp -f ${TARGET}.pdf mm.pdf

arx : ${TARGET}.bbl
	./makex ${ARXIV_DIR} ${ARXIV_FILES}

clean :
	rm -f *.aux *.dvi *.log *.lof *.lot *.toc *.blg *.idx *.out *.tpt

rclean :
	make clean
	rm -f *.ps *.bbl

rrclean :
	make rclean
	rm -f m.pdf mm.pdf ${TARGET}.pdf
	rm -rf ${ARXIV_DIR}


